Keep Your Friends Close, but Your Routeservers Closer: Insights into RPKI Validation in the Internet

IP prefix hijacks allow adversaries to redirect and intercept traffic, posing a threat to the stability and security of the Internet. To prevent prefix hijacks, networks should deploy RPKI and filter bogus BGP announcements with invalid routes. In this work we evaluate the impact of RPKI deployments on the security and resilience of the Internet. We aim to understand which networks filter invalid routes and how effective that filtering is in blocking prefix hijacks. We extend previous data acquisition and analysis methodologies to obtain more accurate identification of networks that filter invalid routes with RPKI. We find that more than 27% of networks enforce RPKI filtering and show for the first time that deployments follow the business incentives of inter-domain routing: providers have an increased motivation to filter in order to avoid losing customers' traffic. Analyzing the effectiveness of RPKI, we find that the current trend to deploy RPKI on routeservers of Internet Exchange Points (IXPs) only provides a localized protection against hijacks but has negligible impact on preventing their spread globally. In contrast, we show that RPKI filtering in Tier-1 providers greatly benefits the security of the Internet as it limits the spread of hijacks to a localized scope. Based on our observations, we provide recommendations on the future roadmap of RPKI deployment. We make our datasets available for public use [https://sit4.me/rpki].

==> readme.tex <==
\section{{\tt README}}\label{ap.sc.readme}
Our datasets are on dropbox account of an anonymous user John Doe: \url{https://www.dropbox.com/s/3zr7sjkyhdrdnap/rov-2022.tar.gz?dl=0} 
\ignore{
The code calculates and prints our classification results. For executing our code please install the following requirements:

{\scriptsize 
\begin{verbatim}
pip install ripe.atlas.cousteau
pip install ripe.atlas.sagan
pip install pycountry_convert
mkdir measured    
\end{verbatim}
}

The data are downloaded on the fly from the primary persistent sources on RIPE Atlas.
% * change reload to True in util.py : ask_asn()
% * run the Jupyter Notebook
% * then change the reload=False back to speed up following runs


}
